Adaptive Constraint Satisfaction for Markov Decision Process Congestion Games: Application to Transportation Networks

Under the Markov decision process (MDP) congestion game framework, we study the problem of enforcing population distribution constraints on a population of players with stochastic dynamics and coupled congestion costs. Existing research demonstrates that the constraints on the players' population distribution can be satisfied by enforcing tolls. However, computing the minimum toll value for constraint satisfaction requires accurate modeling of the player's congestion costs. Motivated by settings where an accurate congestion cost model is unavailable (e.g. transportation networks), we consider an MDP congestion game with unknown congestion costs. We assume that a constraint-enforcing authority can repeatedly enforce tolls on a population of players who converges to an $\epsilon$-optimal population distribution for any given toll. We then construct a myopic update algorithm to compute the minimum toll value while ensuring that the constraints are satisfied on average. We analyze how the players' sub-optimal responses to tolls impact the rates of convergence towards the minimum toll value and constraint satisfaction. Finally, we construct a congestion game model for Uber drivers in Manhattan, New York City (NYC) using data from the Taxi and Limousine Commission (TLC) to illustrate how to efficiently reduce congestion while minimizing the impact on driver earnings.

==> append/A1.tex <==
\begin{lemma}\label{lem:subgradient}
The augmented cost function given by~\eqref{eqn:incentiveCosts}, equivalently written as
\[
\bar{\ell}_{tsa}(y) = \ell_{tsa}(y) + \sum_{z \in \mc{Z}} \tau_z g_z(y),
\]
where $\mc{Z} = \{i \in [I] \ | \ \sum_{t,s,a} A_{tsa}(i)y_{tsa} - b(i) > 0 \} $, is a subgradient of the potential function $F(y)$~\eqref{eqn:tolled_potential}. 
\end{lemma}
\begin{proof}
We consider the extended real-valued function
\[G(y) = \begin{cases}
F(y) & y \in \mc{Y}(P,p), \\
\infty & \text{otherwise}.
\end{cases}\]
The subdifferential set $\partial G(y)$~\cite[App.B.21]{bertsekas1999nonlinear} is defined for all $y \in \mc{Y}(P, p)$ and is given by \[\{g \ | \ G(y') \geq G(y) + g^\top(y' - y), \ \forall \ y' \in \reals^{(T+1)\times S\times A} \}.\]
We now show that $\bar{\ell}(y) \in \partial G(y)$. 
\begin{align}
     &G(y) + \sum_{t,s,a}\bar{\ell}_{tsa}(y)(y_{tsa}' - y_{tsa}) \\ 
   = & F_0(y) + \sum_{i}\tau_i(\sum_{t,s,a}A_{tsa}(i) y_{tsa} - b(i))_+ \notag\\
   & + \sum_{t,s,a}(\ell_{tsa}(y) + \sum_{z} \tau_z A_{tsa}(z))(y_{tsa}' - y_{tsa}) 
\end{align}
% \\
%   = &\sum_{t,s,a} \int_{0}^{y_{tsa}} \ell(u) \partial u +  \sum_{i} \tau_i(\sum_{t,s,a}A_{tsa}(i) y_{tsa} - b(i))_+ \notag\\
%   & + \sum_{t,s,a}\bar{\ell}_{tsa}(y)(y'_{tsa} - y_{tsa})\\ 
%   = & \sum_{t,s,a} \int_0^{y_{tsa}}
Since the original game~\eqref{eqn:mdpcg} is a potential game and $F_0(y)$ has exact gradient $\ell(y)$, $F_0(y)$ satisfies
\begin{align}\label{eqn:a7}
   F_0(y') \geq F_0(y) + \sum_{t,s,a} \ell_{tsa}(y)(y'_{tsa}  - y_{tsa}). 
\end{align}
Therefore to prove that $\bar{\ell}(y) \in \partial G(y)$, we consider $G(y) + \sum_{t,s,a}\bar{\ell}_{tsa}(y)(y_{tsa}' - y_{tsa}) - F_0(y) - \sum_{t,s,a} \ell_{tsa}(y) (y'_{tsa} - y_{tsa})$, given by 
\begin{align}\label{eqn:a3}
     &\sum_{z}\tau_z(\sum_{t,s,a}A_{tsa}(z)(y'_{tsa} - y_{tsa})) \notag \\
     + &\sum_{i}\tau_i(\sum_{t,s,a}A_{tsa}(i) y_{tsa} - b(i))_+,
\end{align}
Since $\mc{Z}$ is the precisely the set of constraints where $\sum_{tsa}A_{tsa}(i) y_{tsa} - b(i) > 0$, \eqref{eqn:a3} evaluates to
\begin{align}\label{eqn:a4}
    \sum_{z \in \mc{Z}} \tau_z \Big(\sum_{t,s,a} A_{tsa}(z) y'_{tsa} - b(z)\Big),
\end{align}
We note that for each $z \in \mc{Z}$, if $\sum_{t,s,a} A_{tsa}(z) (y'_{tsa} - b(z)) < 0 $, we can remove index $z$ from summation and obtain a greater sum, therefore, \eqref{eqn:a4} is less than or equal to 
\begin{align}\label{eqn:a5}
   \sum_{z \in \mc{Z}} \tau_z \Big(\sum_{t,s,a} A_{tsa}(z) y'_{tsa} - b(z)\Big)_+.
\end{align}
Since $\mc{Z} \subseteq [I]$, \eqref{eqn:a5} is less than or equal to
\begin{align}\label{eqn:a6}
    \sum_i \tau_i\Big(\sum_{t,s,a} A_{tsa}(i) y'_{tsa}- b(i)\Big)_+
\end{align}
Finally, we note that~\eqref{eqn:a6} is equivalent to  $G(y') - F_0(y')$ and~\eqref{eqn:a4} is equivalent to $G(y) + \sum_{t,s,a}\bar{\ell}_{tsa}(y)(y_{tsa}' - y_{tsa}) - F_0(y) - \sum_{t,s,a} \ell_{tsa}(y) (y'_{tsa} - y_{tsa})$, therefore
\begin{align}
    G(y') - F_0(y') \geq & G(y) + \sum_{t,s,a}\bar{\ell}_{tsa}(y)(y_{tsa}' - y_{tsa}) - F_0(y) \notag\\
    & - \sum_{t,s,a} \ell_{tsa}(y) (y'_{tsa} - y_{tsa})
\end{align}
From~\eqref{eqn:a7}, it follows that
\[G(y') \geq G(y) + \sum_{t,s,a}\bar{\ell}_{tsa}(y)(y_{tsa}' - y_{tsa}), \ \forall y' \in \reals^{(T+1)\times S\times A} \]
Therefore $\bar{\ell}(y)$ is a subdifferential of $G(y)$ for any $y \in \mc{Y}(P,p)$.
\end{proof}

==> exactPenaltyToll.tex <==
Instead of searching over all possible tolling functions, we assume that the game designer controls $I$ tolling functions to enforce $I$ design constraints, where each tolling function $g_i$ is given by
\begin{equation}\label{eqn:tolls}
g_i(y) = 
\begin{cases}
A(i) & \underset{t,s,a}{\sum}A_{tsa}(i)y_{tsa} - b(i) > 0 \\
0 & \text{otherwise}
\end{cases}. %\quad \forall\ i \in [I].(
\end{equation}
Toll $g_i(y)$ is activated when the $i^{th}$ constraint becomes violated. Furthermore, the toll only affects $(t,s,a)$ where $A_{tsa}(i) > 0$, and its magnitude is proportional to the tolling value $\tau_i$. Parameter $\tau_i \in \reals_+$ is a game designer-controlled parameter. The toll functions change decision maker's costs as
\begin{equation}\label{eqn:incentiveCosts}
    \bar{\ell}(y) = \ell(y) + \sum_i  \tau_i g_i(y).
\end{equation}
 
By adding tolls $\sum_{i}\tau_ig_i$, $\bar{\ell}_{tsa}$ is no longer a continuous function of $y_{tsa}$. As such, Assumption~\ref{assump:decreasing} no longer applies and the game with cost~\eqref{eqn:incentiveCosts} no longer corresponds to a potential game given by~\eqref{eqn:mdpcg_general}. We next show that the MDP congestion game with cost $\bar{\ell}$ does indeed generate a potential game with an optimization formulation, and the solution of said optimization problem is the MDP Wardrop equilibrium of an almost everywhere identical function to $\bar{\ell}$, and under mild assumptions, has a non-empty MDP Wardrop equilibria set. 

==> notation.tex <==
\section{Preliminaries and Background} \label{sec:prelim}
In this section, we present an overview of mathematical preliminaries relevant to MDP congestion games. 

\noindent\textbf{Notation.} We use the notation $[K]=\{0, \ldots, K-1\}$ to denote an index set of length $K$, $\reals$ to denote the set of real numbers, and $\reals_+$ for the set of positive real numbers including zero. For any tensor $Z \in \reals^{N_1\times N_2 \times N_3}$, we use $Z_{n_1 n_2 n_3}$ to denote its components. To denote a vector of ones of size $N$, we use $\ones_N$. The function $g(x) = (x)_+$ outputs $x$ when $x > 0$ and $0$ otherwise.

\subsection{MDP}
We consider the dual of the linear programming formulation of a finite horizon MDP~\cite[Sec.6.9.1]{puterman2014markov} with horizon of length $T$, finite state space $[S]$ and finite action space $[A]$ given by 
\begin{equation}\label{eqn:mdp}
\begin{aligned}
\underset{y}{\min} & \ \underset{t,s,a}{\sum} y_{tsa}c_{tsa} \\
\text{s.t. } &  \sum_{a} y_{0sa}  = p_s, \forall \ s  \in [S], \\
&\sum_a y_{t+1,sa} = \sum_{s',a}P_{tss'a}y_{ts'a},\  \forall t \in [T],\  s \in [S], \\
& y \in \reals_+^{(T+1)\times S \times A}.
\end{aligned}
\end{equation}
The objective is to minimize the total expected cost over the finite time horizon $[T+1]$. 
% The optimization variable $y$ defines a time-varying state-action probability distribution, such that $y_{tsa}/\sum_{a' \in [A]}y_{tsa'}$ denotes a decision maker's probability of taking action $a$ at state $s$ and time $t$. 
The optimization variable $y$ defines a time-varying state-action probability distribution. 
In connection with a time-varying \emph{policy}, $\pi_t: [S] \times [A] \rightarrow [0,1]$, which denotes the probabilistic distribution that a decision maker will take action $a$ from state $s$,  $y_{tsa} = x_t(s)\pi_t(s,a)$, where $x_t \in \reals^{S}$ is the probability distribution of the decision maker at time $t$. From this perspective, $y$ encodes both the probability that a decision maker will be at state $s$ and the likelihood he will take action $a$ from state $s$. 

The probability kernel $P$ defines the MDP transition dynamics, where $P_{tss'a}$ denotes the time varying transition probability from state $s'$ to $s$ when taking action $a$. 
The kernel $P$ satisfies
\[ \sum_{s' \in [S]}P_{ts'sa} = 1, \ P_{ts'sa}\geq 0 \quad \forall\ s', s \in [S], \ a \in [A] ,\  t \in [T].\]
The cost parameter $c_{tsa}$ denotes the cost of taking action $a$ from state $s$ at time $t$. The initial condition is given as $p_{s}$, the probability density at state $s$ at $t = 0$. 
% Solutions to a finite horizon MDP problem described by~\eqref{eqn:mdp} can be obtained using Algorithms~\ref{alg:valueIteration} and \ref{alg:policy iteration}~\cite{altman1999constrained}. Algorithm~\ref{alg:valueIteration} iteratively evaluates the Bellman equation temporally backwards to determine the optimal expected cost-to-go, $V_{ts}$ and the optimal policy, $\pi_{ts}$, which determines the optimal action to take at time $t$ and state $s$. Note the $\min$ operator in Algorithm~\ref{alg:valueIteration} returns two values: the minimum value of the input set, assigned to $V_{ts}$, and the argument of the minimum value, assigned to $\pi_{ts}$.

\subsection{MDP Congestion Game}
An MDP congestion game is played by a continuous population of decision makers, where each has MDP dynamics given by~\eqref{eqn:mdp} with identical cost $c$, identical kernel $P$, and identical initial probability density $p$. 

The \emph{population distribution} is given by  $y \in \reals^{(T+1) \times S\times A}$, such that $y_{tsa}$ is the population density taking action $a$ at state $s$ and time $t$. Because decision makers undergo identical stochastic transition described by kernel $P$, and have the same initial probability density $p$, the set of \emph{feasible} population distributions $\mc{Y}(P,p)$ is described by 
\begin{equation}
    \begin{aligned}\label{eqn:feasibleY}
    \mc{Y}(P,p)  = \{y \in \reals_+^{(T+1)S A}\Big| \, &
    \underset{a}{\sum} y_{t+1,sa} =  \underset{s',a}{\sum}P_{tss'a}y_{ts'a}, \\
    & \underset{a}{\sum}y_{0sa} = p_s \}.
    \end{aligned}
\end{equation}
We say the population has mass $M$ if $\sum_{s \in[S]} p_s = M > 0$. 

The cost of a non-atomic MDP congestion game is identical for each decision maker, but varies with the population distribution as given by 
\begin{align}
c_{tsa} = \ell_{tsa}(y), 
\label{eqn:congestionCosts}
\end{align}
where $\ell_{tsa}:\reals^{(T+1)SA} \rightarrow \reals$. We use $\ell(y) \in \reals^{(T+1)SA}$ to denote the cost vector whose $(t,s,a)$ element is $\ell_{tsa}(y)$. 

\begin{remark}
By considering congestion cost as a function of state-action distribution $y$, MDP congestion games markedly differ from stochastic games, which assume that the cost is a function of policy $\pi$. This difference allows MDP congestion games to model congested stochastic networks more accurately. Stochastic games assign a high cost to state-action pair $(s,a)$ when a group of decision makers take action $a$, yet this congestion cost is superfluous if the decision makers have a low probability of being in state $s$. In contrast, MDP congestion games only assign a high cost when decision makers take a $a$ from state $s$ and have a high probability of arriving at state $s$. 
\end{remark}

When individual decision makers optimize MDPs with state-action costs given by~\eqref{eqn:congestionCosts}, a stable equilibrium reached if, at the current game costs, no decision maker has an incentive to switch to another strategy. We denote this population distribution as an MDP Wardrop equilibrium. 
\begin{definition}[MDP Wardrop Equilibrium \cite{calderone2017markov}]\label{def:wardrop}
A population distribution $y^\star$ is an MDP Wardrop equilibrium if it satisfies
\begin{align}\label{eqn:wardropDef}
 \underset{t,s,a}{\sum} y_{tsa}^\star\ell_{tsa}(y^\star) \leq  \underset{t,s,a}{\sum} y_{tsa}\ell_{tsa}(y^\star), \quad \forall \ y \in \mc{Y}(P,p)
\end{align}
We denote the set of $y^\star \in \mc{Y}(P,p)$ that satisfies~\eqref{eqn:wardropDef} by  $\mc{W}(\ell)$.
\end{definition}
When game designer interacts with a game in which players themselves undergo learning algrithms to reach the Wardrop equilibria, it is often the case that players only reach an $\epsilon-$Wardrop equilibrium in finite time. 
\begin{definition}[$\epsilon$-MDP Wardrop equilibria]
A population distribution $\hat{y}$ is an $\epsilon$-MDP Wardrop equilibrium if it satisfies
% the improvement in expected cost for switching to a different strategy $y \in \mc{Y}(P,p)$ is less than $\epsilon$.
\begin{align}\label{eqn:eWardropDef}
\hat{y}^\top(\ell(\hat{y}) - \epsilon) \leq y^\top(\ell(\hat{y}) - \epsilon), \quad \forall  \ y \in \mc{Y}(P,p) .  
\end{align}
We denote the set of $\hat{y} \in \mc{Y}(P,p)$ that satisfies~\eqref{eqn:eWardropDef} by $\mc{W}(\ell, \epsilon)$.
\end{definition}
The $\epsilon$-Wardrop equilibrium $\hat{y}$ achieves near-optimal costs $\ell(y^\star)$ by an error bound of $\epsilon$ in the sense that by moving to a different distribution, decision maker can decrease its cost by no more than $\epsilon$ in each $(t,s,a)$ triplet. For strongly convex and strongly smooth costs, we show that $\epsilon$ Wardrop equilibria translates directly to a bound on the cost $\ell(\hat{y})$ from the optimal cost $\ell(y^\star)$.
\begin{proposition}\label{prop:epsWE}
If the cost function $\ell$ is $\alpha$ strongly convex and $\beta$ strongly smooth, then for any $\epsilon$ Wardrop equilibrium $\hat{y} \in \mc{W}(\ell, \epsilon)$, 
\[\norm{\ell(\hat{y}) - \ell(y^\star)}_2 \leq \frac{\beta}{\alpha}\norm{\epsilon}_2.\]
\end{proposition}
\begin{proof}
From definition of $\epsilon$-Wardrop equilibrium, we have~\eqref{eqn:eWardropDef} holding for any $y \in \mc{Y}(P, p)$. In particular, it holds for the optimal Wardrop equilibrium $y^\star \in \mc{W}(\ell, 0)$ --- i.e. 
\begin{equation}\label{eqn:prop2_1}
    \ell(\hat{y})^\top(\hat{y} - y^\star) \leq (\epsilon^k)^\top(\hat{y} - y^\star).
\end{equation}
Since $y^\star$ is a Wardrop equilibrium for $\ell$, $\ell(y^\star)^\top(\hat{y} - y^\star) \leq 0 $ follows from~\eqref{eqn:wardropDef}. We add this to the left hand side of~\eqref{eqn:prop2_1}. On the right hand side, bound $(\epsilon^k)^\top(\hat{y} - y^\star)$ by $\norm{\epsilon^k}_2\norm{\hat{y}-y^\star}_2$ to obtain 
\begin{equation}
    (\ell(\hat{y}) - \ell(y^\star))^\top(\hat{y} - y^\star) \leq \norm{\epsilon^k}_2\norm{\hat{y}-y^\star}_2
\end{equation}
$\ell$ is strongly convex by assumption with coefficient $\alpha$. This implies $\alpha \norm{\hat{y} - y^\star}^2_2 \leq (\ell(\hat{y}) - \ell(y^\star))^\top(\hat{y} - y^\star)\leq \norm{\epsilon^k}_2\norm{\hat{y}-y^\star}_2$. $\ell$ is also strongly smooth by assumption with coefficient $\beta$. Strong convexity and strong smoothness together implies the following bound,
\begin{equation}
  \norm{\ell(\hat{y})  - \ell(y^\star)}_2 \leq \beta\norm{\hat{y} - y^\star}_2 \leq \frac{\beta}{\alpha} \norm{\epsilon^k}_2. 
\end{equation}
Therefore the proposition follows. 
\end{proof}

\noindent\textbf{Potential game formulation}. If $\ell(y)$ are continuous functions and an explicit potential function $F: \reals^{(T+1)\times S \times A} \rightarrow \reals$ exists such that $\nabla_y F(y) = \ell(y)$, then MDP congestion games are a subset of \emph{potential games}~\cite{monderer1996potential}. Given a known potential function $F$, all solutions to the following optimization problem are Wardrop equilibria of the corresponding MDP congestion game~\cite{calderone2017markov}:
\begin{equation}\label{eqn:mdpcg_general}
\begin{aligned}
\mc{W}(\ell) = \underset{y}{\argmin} &\,F(y)  \\
\text{s.t. } & y \in \mc{Y}(P,p).
\end{aligned}
\end{equation}
There are many classes of cost function $\ell$ that give rise to potential functions. For example, if  the decision maker's cost function $\ell_{tsa}$ is a continuous function of $y_{tsa}$, the potential function is given by $F_0(y) = \underset{t,s,a}{\sum} \int_{0}^{y_{tsa}}\ell_{tsa}(u) \partial u $. 
% In particular, the optimization problem given by~\eqref{eqn:mdpcg_general} can be re-formulated as
% \begin{equation}\label{eqn:mdpcg}
% \begin{aligned}
% \mc{W}(\ell) = \underset{y}{\argmin} &\,\underset{t,s,a}{\sum} \int_{0}^{y_{tsa}} \ell_{tsa}(u) \partial u \\
% \text{s.t. } & y \in \mc{Y}(P,p).
% \end{aligned}
% \end{equation}
Furthermore, the following assumption on the cost $\ell$ renders~\eqref{eqn:mdpcg_general} a convex optimization problem~\cite{calderone2017markov}. 
\begin{assumption}[Monotonicity]
\label{assump:decreasing}
For each $y', y \in \mc{Y}(P,p)$, $y_{tsa}' \geq y_{tsa}$, the $(t,s,a)$ element of cost vector $\ell(y)$ is continuous and satisfies $\ell_{tsa}(y_{tsa}') \geq \ell_{tsa}(y_{tsa})$, for all $(t,s,a) \in [T+1]\times [S]\times [A]$.
\end{assumption}
\begin{remark}
Analogous to the colloquial meaning of congestion, Assumption~\ref{assump:decreasing} states that the state-action cost for triplet $(t,s,a)$ cannot decrease as the population density that chooses it increases. A limiting scenario is the classic finite time horizon MDP given by~\eqref{eqn:mdp}, in which $\ell_{tsa} = c_{tsa}$. 
\end{remark}

As a convex optimization problem, the solution set $\mc{W}(\ell)$ is a convex set, and in general is not unique. The convex potential formulation of an MDP congestion game allows us to leverage existing convex optimization techniques to find MDP Wardrop equilibria. In particular, the Frank-Wolfe algorithm combined with dynamic programming techniques for MDPs is an efficient gradient-descent algorithm for determining the Wardrop equilibrium population distribution~\cite{us,yu2019primal}. By leveraging dynamic programming to compute linearized subproblems, the Frank-Wolfe algorithm is a more efficient method than off the shelf convex optimization solvers for lower precision requirements. Furthermore, the algorithm also has a natural online interpretation in the repeated game setting: by independently updating its actions based on previous game's costs, the continuous population of decision makers collectively converge to the Wardrop equilibrium~\cite{us}. 
% if tolling algorithm is the same, take this last bit out
% We outline the algorithm in Algorithm~\ref{alg:FrankWolfe}. 
% \begin{algorithm}
% \caption{Frank-Wolfe for MDP Congestion Game}
% \begin{algorithmic}[1]
% \Require \(\ell\), \(P\), \(p\), \(N\), \(\epsilon\).
% \Ensure \(y^{\star}\).
% \State{\( y^0 = 0 \in \reals^{(T+1)\times S\times A} \)}
% \For{\(k = 1, 2, \ldots, N\)}\label{alg:fw_kStart}
%     \State{\(c^k = \ell(y^{k-1}) \)}\label{alg:fw_costEval} %+ \underset{i\in\mc{I}}{\sum}\tau_i g_i(y^k)
%     \State{\( \alpha^k =  \frac{2}{k+1} \)}
% 	\State{\( \pi^{k} = \) \Call{Backward Induction}{$c^k, P$}}\label{alg:fw_polIter}	\Comment{Alg.~\ref{alg:valueIteration}}
% 	\State{\(d^k\) = \Call{Forward Induction}{$P, p, \pi^{k}$}}\label{alg:fw_gamePlay}\Comment{Alg.~\ref{alg:policy iteration}}
% 	\State{\( y^k = (1 - \alpha^k)y^{k-1} + \alpha^k d^k\)} \label{alg:fw_policyChange}
% 	\State{Stop if \(q(y^k) \leq \epsilon\)}
% \EndFor\label{alg:fw_kEnd}
% \end{algorithmic}
% \label{alg:FrankWolfe}
% \end{algorithm}



==> simulation_no_queue.tex <==
\section{Congestion Reduction in Ride-share Networks}~\label{sec:ny_rideshare}
\noindent In this section, we model the competition among NYC's ride-share drivers as a MDP congestion game and apply Algorithm~\ref{alg:dualAscent} to demonstrate how ride-share companies can implicitly enforce constraints by utilizing tolls. 
Since origin-destination-specific trip data for ride-share companies are not publicly available, we use the rider demand distribution provided by the NYC TLC as a proxy for Uber's rider demand distribution. In~\cite{taxi_frequency}, the overall rider demand for TLC is estimated to be about $40\%$ of the rider demand for Uber. \ctwo{We assume that TLC's ride demand accurately estimates Uber's ride demand up to scaling and normalize accordingly.}
\subsection{Ride-sharing MDP} 
We consider a cohort of competitive ride-share drivers in Manhattan, NYC repeatedly operating between $9$ am and noon.Using over six hundred thousand data points from the yellow taxi data during January, 2019~\cite{new_york_taxi}, we model individual driver dynamics as a finite time horizon MDP. 

\change{
\noindent\textbf{Modeling assumptions}. 1) \ctwo{We assume that all trips take discretized times of $[15, 20, 30,\ldots]$ determined by origin to destination distance. 2) In the following section, we assume that the initial driver distribution is uniform}, i.e. $p_s = 10000/63$ for each $s \in [S]$. We find that varying the initial distribution did not significantly impact the time-averaged MDP Wardrop equilibrium or the approximate norm of the resulting tolls, as long the initial distribution does not violate constraints.  3) From~\cite{uber_driver_density}, the Uber driver population in NYC is approximately $50 000$. We assume that $20\%$ of the total population works in Manhattan between $9$ am and noon. 
}

\noindent\textbf{States}. As shown in Figure~\ref{fig:manhattan_taxi_zones}, Manhattan is discretized into $63$ states that correspond to TLC's taxi zones (excluding the island zones).  \change{For state $s$, its neighboring states are those geographically adjacent (sharing one or more edges) to $s$ in Figure~\ref{fig:manhattan_taxi_zones}.} The set of neighbors is denoted by $\mc{N}(s)$.

\noindent\textbf{Actions}. 
\change{Actions are state-specific. Two action types are available at $s \in [S]$. Action $a_{s'}$ for any $s' \in \mc{N}(s)$ transitions the driver from $s$ to $s'$. Action $a_s$ signals that the driver will stay in state $s$ and wait for a rider. At $(s, a_s)$, we assume drivers will always find a rider (but will be deterred by congested costs). The total number of available actions for all states is given by} \[A = 1 + \max_{s \in [S]} | \mc{N}(s)|.\] 
We use $|\mc{N}(s)|$ to denote the number of neighbors of state $s$. Each action $a_i \in [A]$ corresponds to different actions for different states. In states with less neighbors than $\max_{s} | \mc{N}(s)|$, the extra actions are repeats of previous actions.  For example, for state $1$ with neighbors $\{3\}$, the available actions are $\{a_1, a_3, a_3\}$. For state $2$ with neighbors $\{3, 4\}$, the available actions are $\{a_2, a_3, a_4\}$. 

\noindent\textbf{Time.} The average trip time from the TLC data is $12.02$ minutes. Therefore, we take $12$ minutes time intervals between $9$ am and noon for a total of $T = 15$ time steps. 

\noindent\textbf{Transition Dynamics.}
% The initial driver distribution $p$ is assumed to be uniform, i.e. $p_s = 10000/63$ for each $s \in [S]$. 
For action $a_{s'}$ from state $s$ at time $t$, the transition probability to any state $\bar{s}$ is given by 
\begin{equation}
    P(s, a_{s'}, \bar{s}, t) =
    \left\{\begin{array}{ll}
  1 - \delta, & \text{if}\ \bar{s} = s',\\
  \frac{\delta}{| \mc{N}(s) | - 1}, & \text{if}\ \bar{s} \neq s',\ \bar{s} \in \mc{N}(s),\\
  0,& \text{otherwise},
  \end{array}\right. \notag
\end{equation}
where $\delta \in [0,1)$ models the driver's probability of real-time deviation from a chosen strategy. We set $\delta = 0.1$.

\change{For action $a_s$ from state $s$ at time $t$, the transition probabilities to any state $\bar{s}$ is derived using the rider demand distribution at $s$. Let $N(s, \bar{s}, t)$ be the number of trips with origin-destination $(s, \bar{s})$ at time step $t$.} The transition probability to state $\bar{s}$ is given by
\[\textstyle P(\bar{s}, s, a_{s}, t) = \frac{N(s, \bar{s}, t)}{\sum_{s'} N(s, s', t)}, \quad \forall \ \bar{s} \in [S], \ t \in [T].\]
\change{
Note that $a_s$ may transition drivers to states outside of $\mc{N}(s)$.}

\noindent\textbf{Driver costs}. As in~\cite{us}, the driver cost is the sum of expected earnings, fuel cost, and an artificial congestion cost.
\begin{align}
\ell_{tsa}(y_{tsa}) & =\mathbb{E}_{s'} \left[c_{ts's}^\text{trav} - m_{ts's} \right] + c_{t}^\text{wait}\cdot y_{tsa} \notag \\
& = \textstyle\sum_{s'}P_{ts'sa}\left[ c_{ts's}^\text{trav} -m_{ts's}\right] + c_{t}^\text{wait}\cdot y_{tsa} \notag
\end{align}
where $m_{ts's}$ is the monetary reward that the driver receives for transitioning from state $s$ to $s'$ (only available when $a = a_s$), $c_{ts's}^\text{trav}$ is the fuel cost of travelling from state $s$ to $s'$, $c_{t}^\text{wait}$ is the coefficient of congestion, scaled linearly by the portion of drivers who are waiting for a rider. For a trip time of $\Delta t$, the cost of UberX in NYC~\cite{uber_pricing} is given by
\begin{equation}\label{eqn:trip_costs}
 m_{ts's} = \max\Big( \$ 7, \$ 2.55  + \$ 0.35 \cdot \Delta t \text{(min)} + \$ 1.75 \cdot \Delta d \text{(mi)}\Big).
\end{equation}
To compute $m_{ts's}$, we assign $\Delta t = 12$ minutes  and $\Delta d = d_{ss'}$ as the Haversine distance from $s$ to $s'$ in miles. If $s' = s$, we average existing TLC data for $(s, s)$ trips estimate $d_{ss}$. Other parameters of $\ell_{tsa}$ are computed as 
\begin{subequations}
\begin{align}
c_{ts's}^\text{trav} & = 
\mu
\underbrace{d_{ss'}}_{\text{mi}}
\underbrace{\big(\text{Vel}\big)^{-1}}_{\text{hr}/\text{mi}} + 
%}_{\text{Time Cost}} 
\underbrace{\big(\substack{\text{Fuel} \\ \text{Price} } \big)}_{\$/\text{gal}}
\underbrace{\big( \substack{\text{Fuel} \\ \text{Eff}} \big)^{-1}}_{\text{gal}/\text{mi}} 
\underbrace{d_{ss'}}_{\text{mi}} \\
c^\text{wait}_{tsa} & = 
\begin{cases}
\underset{s'}{\mathbb{E}}\left[m_{ts's}\right] \cdot 
\Big(%\frac{1}{
\underbrace{
\substack{\text{Customer} \\ \text{Demand Rate} }%}
}_{\text{rides}/\Delta t}
\Big)^{-1}, & \text{ if $a=a_s$} \\
\omega_{tsa_{s'}}, & \text{ if $a=a_s'$}
\end{cases}
\label{eq:travel}
\end{align}
\end{subequations}
where $\mu$ is a time-money tradeoff parameter,  $\omega_{tsa_{s'}} = 0.1$ models the minor congestion effects for Uber drivers who decide to traverse from $s$ to $s'$. 

The customer demand rate is derived from TLC data per time interval per day. We estimate Uber ride demand to be 2.5 times more than the Yellow Taxi's ride demand in January 2019~\cite{uber_vs_taxi_demand} and scale the TLC ride data accordingly. 
Other parameter values are listed in Table~\ref{tab:params}. 
\begin{table}[h!]
\begin{center}
\begin{tabular}{|cccc|}
\hline
$\mu$  & Velocity & Fuel Price & Fuel Eff   \\
\hline
\$15 /mi & 8 mph & \$2.5/gal & 20 mi/gal \\
\hline
\end{tabular}
\caption{Parameters for the driver cost function.}\label{tab:params}
\end{center}
\end{table}
\subsection{Online learning via conditional gradient descent}
In the previous section, we built a MDP congestion game model for the purpose of simulating Manhattan's ride-share game. 
We assume that the players cannot directly access the congestion costs model and transition dynamics. Instead, drivers collectively receive costs for a chosen joint policy, and iteratively find the MDP Wardrop equilibrium. 

We implement the learning method from~\cite[Alg.3]{us}. Inspired by conditional gradient descent (Frank-Wolfe), this method implicitly enforces $y \in \mc{Y}(P, p_0)$ by solving the linearized objectives via dynamic programming. Although conditional gradient descent can be slow to converge to higher accuracy, it converges faster to lower accuracy solutions. From the stopping criterion for conditional gradient descent, we compute $\epsilon$ for the $\epsilon^k$-MDP Wardrop equilibrium as 
\begin{equation}\label{eqn:manhattan_stopping_criterion}
  \textstyle\epsilon^k = \big(\ell(y^k) + A^\top\tau^k\big)^\top(y^k - y^{k+1}). 
\end{equation} 
\begin{figure}
    \centering
    \includegraphics[width=1.08\columnwidth]{figs/manhattan_unconstrained_combo.pdf}
    \caption{Predicted ride-share traffic in Manhattan.}
    % for $10000$ drivers. The map plot shows the predicted driver distribution averaged over $15$ time steps. The bar plot and the line plot displays the constraint violation in the most highly congested states~\eqref{eqn:manhattan_constraints}.}
    \label{fig:manhattan_taxi_zones}
\end{figure}

We set $\epsilon^k = 2e^3$, which is approximately equivalent to a normalized error of $1\%$ for the game potential $F_0$~\eqref{eqn:integral_potential}. The corresponding $\epsilon$-MDP Wardrop equilibrium as well as the time-averaged/varying driver densities of the most congested states are shown in the map/line/bar plot in Figure~\ref{fig:manhattan_taxi_zones}. 

From Figure~\ref{fig:manhattan_taxi_zones}, we see that the three most congested zones are the red zones on the bottom-left and center of Manhattan. 
% This correlates well with the congestion results from the NYC Department of Transportation's analysis of taxi speeds~\cite[Pg.13]{nyc_dot}, where the highest congestion levels occur in similar regions. We can infer that our MDP congestion model reasonably approximates the actual behaviour of ride-share drivers. 
Interestingly, our simulation shows that they attract $13\%$ of the working driver population This further motivates the need to reduce congestion within ride-share drivers. 

\subsection{Reducing driver presence in congested taxi zones}
\change{
Using Algorithm~\ref{alg:dualAscent}, ride-share companies can reduce the driver presence in the congested taxi zones without constraining driver behaviour or significantly impacting driver earnings. Suppose the ride-share company wishes to reduce the driver presence to less than $400$ per zone per time.} This constraint can be formulated as
\begin{figure}
    \centering
    \includegraphics[width=0.88\columnwidth]{figs/manhattan_constrained_combo.pdf}
    \caption{Manhattan game with constraints~\eqref{eqn:manhattan_constraints} enforced. The map plot shows the tolled, time-averaged driver distribution. The top line plot shows congestion tolls (\$). The bottom line plot shows the congested driver distributions. }
    \label{fig:manhattan_tolled}
\end{figure}
\begin{equation}\label{eqn:manhattan_constraints}
    \textstyle\sum_{a} y_{tsa} \leq 400, \quad \ \forall \ (t, s) \in [T+1]\times[S].
\end{equation}
For each $(t,s)$, the corresponding constraint is given by $A_i \in \reals^{(T+1)SA}$, where the $(t,s,a)^{th}$ entry is $1$ and all other entries are $0$.
Although only three states violate the capacity constraint in  Figure~\ref{fig:manhattan_taxi_zones}, we enforce all $(t, s) \in [T+1]\times[S]$ constraints to ensure that no constraint violation results in the final equilibria. Thus, we enforce a total of $63 \times 16 = 1008$ constraints of form~\eqref{eqn:manhattan_constraints}. The constraint matrix is $\textstyle A = [A_1, \ldots, A_{(T+1)S}]^\top \in \reals^{(T+1)S\times (T+1)SA}$. 
\subsection{Discussion}
We run Algorithm~\ref{alg:dualAscent} for $2000$ iterations. The results are shown in Figure~\ref{fig:manhattan_tolled}. When $\epsilon^k$ is about $1\%$ of the unconstrained optimal potential value, the resulting constraint violation is quite low, with less than $5$ driver violations per time step. Furthermore, the tolls required to enforce these constraints do not extend beyond $\$0.15$ per time step for all three states. 

From Figure~\ref{fig:manhattan_system_analysis}(top), we conclude that for a total of less than $\$1$ toll over all states per time step, we can decrease the total constraint violation from over $200$ drivers to less than $5$ drivers for the $4$ hour period. Our tolls amount to $\$3.25$ for spending $4$ hours in the most congested state. This is comparable to the proposed toll value for lower Manhattan ($\$2.25$ per entry)~\cite{nyc_congestion_toll}.  

A major concern for ride-share companies is the tolling effect on driver earnings. \change{Driver earning is proportional to the \emph{social objective}~\cite{us} as opposed to~\eqref{eqn:mdpcg_general} minimized by the game. Under tolling, drivers may quit if their average earnings decrease significantly, thus reducing the ride-share workforce.}
% In general, tolling does not necessarily cause average player earning to decrease~\cite{us}.
% This is because the average player earning can be viewed as the \emph{socially optimal} population distribution, which minimizes a different optimization objective than the game's potential~\eqref{eqn:mdpcg_general}. 
Here, we show empirically that tolling does not significantly impact driver earnings. In Figure~\ref{fig:manhattan_system_analysis}(bottom), we plot the average driver earnings during the tolling process, normalized by the untolled average earnings. We observe that the driver earnings change by less than $0.1\%$ under Algorithm~\ref{alg:dualAscent}. Therefore tolling is unlikely to cause quitting among the drivers under this constraint satisfaction scenario. 
\begin{figure}
\center
\subfloat{\includegraphics[ width=0.9\columnwidth]{figs/manhattan_toll_and_violation.pdf}} \newline
\subfloat{\includegraphics[ width=0.95\columnwidth]{figs/manhattan_social_cost.pdf}} 
\caption{Top: total toll enforced and constraint violation during toll synthesis. Bottom: average driver earnings during toll synthesis.}
    \label{fig:manhattan_system_analysis}
\end{figure}

Next, we investigate the effects of $\epsilon^k$ on the toll value and the average constraint violation. In  Figure~\ref{fig:epsilon_analysis}, we compare the average toll value $\ones^\top\thickbar{\tau}^k$ and the average constraint violation $\ones^\top[A\thickbar{y}^k - b]_+$  after $k = 500$ iterations for $\epsilon = [1e3,\ 2e3,\ 2e4,\ 1e5]$. We see that the increased accuracy in $\epsilon$ decreases both the toll value and the constraint violation during the tolling process, thus providing more incentive to accurately compute the minimum toll value. 
\begin{figure}
\center
\subfloat{\includegraphics[ width=0.5\columnwidth]{figs/epsilon_vs_toll.pdf}} 
\subfloat{\includegraphics[ width=0.5\columnwidth]{figs/epsilon_vs_violation.pdf}}
\caption{Left: average toll. Right: average constraint violation. } %Both figures are obtained for $k=500$ iterations as a function of $\epsilon$ inexact oracles
\label{fig:epsilon_analysis}
\end{figure}

% \subsection{Comparison with fast gradient method}
% \change{
% An alternative solution to Algorithm~\ref{alg:dualAscent} is the fast inexact gradient method from~\cite{devolder2014first}. While the fast inexact gradient method in general is shown to have faster convergence properties, we show that in the tolling setting, the fast gradient method provides faster convergence towards optimal toll but trades-off stability in player's social cost. }

% \change{
% To perform fast gradient descent, we modify Algorithm~\ref{alg:dualAscent} Step~\ref{algline:dual_ascent_tau_update} as
% \begin{multline}
%     \tau_{k+1} = \beta_k [\sum_{i = 0}^k \frac{\alpha_i}{L}  (Ay^k - b)]_+ + (1 - \beta_k) [\tau_k + \gamma^k (Ay^k - b)]_+, \\
%     \beta_k = \frac{\alpha_{k+1}}{A_{k+1}L}, \
%     A_{k+1} = \sum_{i=0}^{k+1} \frac{\alpha_i}{L}. 
% \end{multline}
% The resulting toll values, constraint violations, and drivers' social cost changes is shown in Figures~\ref{fig:fast_toll_constraint_comparison} and ~\ref{fig:fast_social_comparison}, respectively. In terms of the last iterate convergence for both the tolling value and the constraint violation, we note that the algorithm results in significantly higher toll values during the tolling process. This negatively impacts the drivers' social costs, resulting in as much as a $70\%$ decrease over the course of the tolling algorithm. In settings where the tolling algorithm directly interacts with a group of players who have an option to quit the game, such a tolling scheme may turn players away and therefore not viable.
% }
% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.88\columnwidth]{figs/fast_grad/toll_value_convergence.pdf}
% %     \caption{Average/last iterate toll convergence comparison for the (fast) gradient methods.}
% %     \label{fig:fast_toll_comparison}
% % \end{figure}

% \begin{figure}
% \center
% \subfloat{
% \resizebox{0.88\columnwidth}{2cm}{\includegraphics{figs/fast_grad/toll_value_convergence.pdf}}}
% \newline
% \subfloat{
% \resizebox{0.88\columnwidth}{2cm}{\includegraphics{figs/fast_grad/constraint_violation.pdf}}}
% \caption{Top: average/last iterate toll convergence comparison for the (fast) gradient methods. Bottom: average/last iterate constraint violation comparison for the (fast) gradient methods. Bottom: }
% \label{fig:fast_toll_constraint_comparison}
% \end{figure}

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.88\columnwidth]{figs/fast_grad/constraint_violation.pdf}
% %     \caption{Average/last iterate constraint violation comparison for the (fast) gradient methods.}
% %     \label{fig:fast_constraint_violation}
% % \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.88\columnwidth]{figs/fast_grad/social_cost.pdf}
%     \caption{Social cost comparison for the (fast) gradient methods.}
%     \label{fig:fast_social_comparison}
% \end{figure}

% https://ny.curbed.com/2018/1/30/16949732/nyc-congestion-pricing-drivers-impact-



% \change{Other figures needed: total amount of toll enforced, total change in the driver earnings, total change in the company earnings.}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\columnwidth]{figs/incentive_convergence.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\columnwidth]{figs/constraint_violation_convergence.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
